FLAG Review 2021

We review lattice results related to pion, kaon, $D$-meson, $B$-meson, and nucleon physics with the aim of making them easily accessible to the nuclear and particle physics communities. More specifically, we report on the determination of the light-quark masses, the form factor $f_+(0)$ arising in the semileptonic $K \to \pi$ transition at zero momentum transfer, as well as the decay constant ratio $f_K/f_\pi$ and its consequences for the CKM matrix elements $V_{us}$ and $V_{ud}$. Furthermore, we describe the results obtained on the lattice for some of the low-energy constants of $SU(2)_L\times SU(2)_R$ and $SU(3)_L\times SU(3)_R$ Chiral Perturbation Theory. We review the determination of the $B_K$ parameter of neutral kaon mixing as well as the additional four $B$ parameters that arise in theories of physics beyond the Standard Model. For the heavy-quark sector, we provide results for $m_c$ and $m_b$ as well as those for the decay constants, form factors, and mixing parameters of charmed and bottom mesons and baryons. These are the heavy-quark quantities most relevant for the determination of CKM matrix elements and the global CKM unitarity-triangle fit. We review the status of lattice determinations of the strong coupling constant $\alpha_s$. We consider nucleon matrix elements, and review the determinations of the axial, scalar and tensor bilinears, both isovector and flavor diagonal. Finally, in this review we have added a new section reviewing determinations of scale-setting quantities.

==> Makefile <==
quick:
	pdflatex FLAG_master.tex

pdflatex:
	pdflatex FLAG_master.tex
	bibtex FLAG_master
	pdflatex FLAG_master.tex
	pdflatex FLAG_master.tex

M	:
	pdflatex FLAG_master.tex
	bibtex FLAG_master
	pdflatex FLAG_master.tex
	pdflatex FLAG_master.tex
	mv FLAG_master.pdf FLAG.pdf

M0	:
	pdflatex FLAG_master.tex
	mv FLAG_master.pdf FLAG.pdf

S	:
	pdflatex Scalesetting_master.tex
	bibtex Scalesetting_master
	pdflatex Scalesetting_master.tex
	pdflatex Scalesetting_master.tex
	mv Scalesetting_master.pdf FLAG.pdf

S0	:
	pdflatex Scalesetting_master.tex
	dvips -Ppdf -GO Scalesetting_master.dvi -o Scalesetting_master.ps
	mv Scalesetting_master.pdf FLAG.pdf		



SECTIONS =  FLAG_introduction FLAG_criteria FLAG_qmass FLAG_VudVus FLAG_LECs FLAG_BK FLAG_HQD FLAG_HQB FLAG_Alpha_s FLAG_NME FLAG_ScaleSetting FLAG_glossary FLAG_notes 

#
#FLAG_glossary FLAG_notes

FLAGsections: %: ${SECTIONS} 


${SECTIONS}: %: Sections/%.tex 
	pdflatex $<
	bibtex $@
	pdflatex $<
	grep sec FLAG_master.aux >> $@.aux
	grep eq FLAG_master.aux >> $@.aux
	grep foot FLAG_master.aux >> $@.aux

	pdflatex $<
	if [ ! -d Sections_pdf ]; then mkdir Sections_pdf; fi	
	mv  $@.pdf Sections_pdf/	


# make sure first entry is a single-scatter plot (MULTIPLE=0)!!!
qmassFigures = ms mud ratio_msmud ratio_mumd
VudusFigures = fp fKfpi Vusud fKandfpi VusVersusVud
LECFigures = su2_Fpi_F su2_Sigma su2_l3bar su2_l4bar su2_l6bar su3_2L6-L4 su3_2L8-L5 su3_L4 su3_L5 su3_L6 su3_L8
BKFigures = BK
HQFigures = FBratio fBandfBs fBsqrtBB2  BB2 xiandRBB BtoPi BtoDStar Vub Vcb fDandfDs FDratio DtoPiandDtoK VcdandVcs BtoD    
Alpha_sFigures = alphasMSbarZ r0LamMSbar
NMEFigures = 
Plots: qmassPlots VudusPlots LECPlots BKPlots HQPlots NMEPlots ScaleSettingPlots # Alpha_sPlots

compileplots=sh -c '\
	cd $$1/Figures ; \
        pwd;\
	for i in `ls -1 *.py|grep -v FLAGplot`; do \
		pythonw $$i ;\
	done;	\
	cd ../../' compileplots


qmassPlots: 
	${compileplots} qmass

VudusPlots: 
	${compileplots} Vudus

LECPlots:
	${compileplots} LEC

BKPlots:
	${compileplots} BK

HQPlots:
	${compileplots} HQ

Alpha_sPlots:
	${compileplots} Alpha_s

NMEPlots:
	${compileplots} NME

ScaleSettingPlots:
	${compileplots} ScaleSetting


clean   :
	rm *.aux *.bbl *.blg *.dvi *.log *.out *.ps FLAG.pdf




==> NME/Tables/app_actions.tex <==
\begin{table}[h]
\mbox{} \\[-0.5cm]
\footnotesize
\begin{tabular*}{\textwidth}[l] {l @{\extracolsep{\fill}} c c c c }\hline\hline\\[-1.0ex]
 Collab. & Ref. & $N_f$ &  \parbox{1cm}{gauge\\action} &  \parbox{1cm}{quark\\action} \\
&& &&\\[-0.1cm]
\hline
\hline
&& &&\\[-0.1cm]
ETM 15D,16A,17B,17C,17 & \cite{Abdel-Rehim:2015owa,Abdel-Rehim:2016won,Alexandrou:2017hac,Alexandrou:2017oeh,Alexandrou:2017qyt} & 2 & Iwasaki  & tmWil$^{\$}$  \\[0.5ex] 
JLQCD 08B & \cite{Ohki:2008ff} & 2 &  Iwasaki & overlap  \\[0.5ex] 
Mainz 12,17 & \cite{Capitani:2012gj,Capitani:2017qpc} & 2 &  Wilson & npSW  \\[0.5ex] 
QCDSF 06,12,13 & \cite{Khan:2006de,Bali:2012qs,Horsley:2013ayv} & 2 &  Wilson & npSW  \\[0.5ex] 
RBC 08 & \cite{Lin:2008uz} & 2 &  DBW2 & DW  \\[0.5ex] 
RQCD 14,16 & \cite{Bali:2014nma,Bali:2016lvx} & 2 &  Wilson & npSW  \\[0.5ex] 
\hline
$\chi$QCD 13A,15 & \cite{Gong:2013vja,Gong:2015iir} & 2+1 & Iwasaki  & DW$^{\star}$  \\[0.5ex] 
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & Iwasaki  & DW,M-DW$^{\star}$  \\[0.5ex] 
$\chi$QCD 15A & \cite{Yang:2015uis} & 2+1 & Iwasaki  & M-DW$^{\star}$  \\[0.5ex] 
BMW 15 & \cite{Durr:2015dna} & 2+1 &  tlSym & HEX-tlSW  \\[0.5ex] 
BMW 11A & \cite{Durr:2011mp} & 2+1 &  tlSym & stout-tlSW  \\[0.5ex] 
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
JLQCD 12A,18 & \cite{Oksuzian:2012rzb,Yamanaka:2018uud} & 2+1 &  Iwasaki & overlap  \\[0.5ex] 
Junnarkar 13 & \cite{Junnarkar:2013ac} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
LHPC 05,10 & \cite{Edwards:2005ym,Bratt:2010jn} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
LHPC 12,12A & \cite{Green:2012ej,Green:2012ud} & 2+1 &  tlSym & HEX-tlSW  \\[0.5ex] 
MILC 09D,12C & \cite{Toussaint:2009pz,Freeman:2012ry} & 2+1 &  tadSym & Asqtad  \\[0.5ex] 
Mainz 18 & \cite{Ottnad:2018fri} & 2+1 &  tlSym & npSW  \\[0.5ex] 
Martin~Camalich 10 & \cite{MartinCamalich:2010fp} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
PACS 18 & \cite{Ishikawa:2018rew} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
PACS-CS 09 & \cite{Ishikawa:2009vc} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
QCDSF 11 & \cite{Horsley:2011wr} & 2+1 &  tlSym & npSW  \\[0.5ex] 
RBC/UKQCD 08B,09B,10D & \cite{Yamazaki:2008py,Yamazaki:2009zq,Aoki:2010xg} & 2+1 &  Iwasaki & DW  \\[0.5ex] 
Shanahan 12 & \cite{Shanahan:2012wh} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
\hline
CalLat 17,18 & \cite{Berkowitz:2017gql,Chang:2018uxx} & 2+1+1 & tadSym  & HISQ$^{\#}$  \\[0.5ex] 
ETM 14A & \cite{Alexandrou:2014sha} & 2+1+1 & Iwasaki  & tmWil$^{\$}$  \\[0.5ex] 
MILC 12C & \cite{Freeman:2012ry} & 2+1+1 &  tadSym & HISQ  \\[0.5ex] 
PNDME 13,15,16,18B,18A,18 & \cite{Bhattacharya:2013ehc,Bhattacharya:2015wna,Bhattacharya:2015esa,Bhattacharya:2016zcn,Gupta:2018lvp,Lin:2018obj,Gupta:2018qil} & 2+1+1 & tadSym  & HISQ$^{\ddag}$  \\[0.5ex] 
\hline
\hline
\end{tabular*}
\begin{minipage}{\linewidth} 
{\footnotesize 
\begin{itemize} 
 \item[$^{\$}$]  Calculations involving the strange and charm quarks use Osterwalder-Seiler~\cite{Osterwalder:1977pc} fermions for these quark flavours. \\[-5mm]
 \item[$^{\star}$]  The calculation uses overlap fermions in the valence quark sector. \\[-5mm]
 \item[$^{\dagger}$]  The calculation uses DW fermions in the valence quark sector. \\[-5mm]
 \item[$^{\#}$]  The calculation uses M-DW fermions in the valence quark sector. \\[-5mm]
 \item[$^{\ddag}$]  The calculation uses mfSW fermions in the valence quark sector. \\[-5mm]
\end{itemize}
}
\end{minipage}
\caption{Summary of simulated lattice actions for calculations in Sec.~\ref{sec:NME}.
\label{tab:NME lattice actions}}
\end{table}


==> ScaleSetting/Mainztalk.tex <==
%%%%%%%%
\subsection{From Rainer's Mainz proceedings}
\newcommand{\fk}{F_\mathrm{K}}
\newcommand{\prot}{\mathrm{prot}}
\newcommand{\nf}{\Nf}
\def\Rho{{\cal R}}
\def\mlat{m^\mathrm{lat}}
\def\prot{\mathrm{p}}
\def\quark{\mathrm{quark}}
\def\sm{S^\mathrm{m}}
\def\sa{S^\mathrm{a}}
\def\metas{m_{\eta_s}}
\def\texp{\tau_\mathrm{exp}}
\def\tauexp{\tau_\mathrm{exp}}
\def\vud{V_\mathrm{ud}}
\def\vus{V_\mathrm{us}}
\def\expe{{\cal E}}
\def\tauexp{\tau_\mathrm{exp}}
\def\tauint{\tau_\mathrm{int}}
\def\tmc{t_\mathrm{MC}}
\def\mprot{m_\prot}
\def\Mprot{M_\prot}

\subsubsection{Introduction}
Presumably the most natural scale for low energy QCD is 
the mass of the proton, $m_\prot$. It is very well knwown.
Alternatively, as a theorist, one might 
like the pseudo scalar decay constant in the chiral limit, called $f$. 
It sets the scale for interactions of the very low
energy description of QCD.
% by chiral perturbation theory.
Indeed, 
let us consider for a little while just QCD in the chiral limit, 
in order to simplify the discussion. 
In this limit, ratios of pairs of these scales or any
other observables of dimension mass, $m_i$,  are predictions of the
theory, but not the scale itself. The latter, and only it, has to be taken from experiment.
In lattice QCD this manifests itself in the fact that 
dimensionless ratios,
$$
    \Rho_i = m_i / \mprot
$$
can be computed and {\em have a continuum limit}. Taking 
$\mprot$ as a reference here is what we call scale setting.
Equivalently, a lattice computation determines dimensionless
quantities $M_i=m_i a,\; \Mprot=\mprot a$ as a function of the
bare coupling $g_0$. The prediction for the physical, dimensionful quantity, $m_i$ is then obtained by
$$
  m_i = \Rho_i \mprot \,,\quad \Rho_i = 
    \lim_{\Mprot\to0} \frac{M_i}{\Mprot} 
  = \lim_{g_0\to 0} \frac{M_i(g_0)}{\Mprot(g_0)} \,.
$$
In lattice slang, scale setting usually is refered to the 
equivalent point of view of determining the lattice spacing $a$
at a given $g_0$ from the specific quantity $\mprot$,
$$
    a_\prot(g_0) = \frac{\Mprot(g_0)}{\mprot}\,,
$$
with the purpose of then defining any other dimensionful
quantity 
$$
  \mlat_i(g_0) = \frac{M_i(g_0)}{a_\prot(g_0)} \,.
$$
Clearly $\mlat_i(g_0)$ has a continuum limit and 
at finite $g_0$ (finite $a$) it has lattice artifacts 
(deviations from this limit)
which depend also on the choice of scale, $\mprot$. 

In practise, we also approximate QCD by an effective 
theory where heavy quarks are removed (one often says integrated out).
How good this approximation is also depends on the
choice of the scale as is apparent from the previous discussion.



\subsubsection{Scale setting is important}

Why is scale setting discussed in a plenary talk?
Both in planning simulations and in the analysis
of the results, the scale (as explained above, whether I say the 
scale or the lattice spacing is just the same) is usually very important.
When quark masses are neglected, an error made in the
scale, systematic or statistical, propagates linearly into a 
hadron mass. 

Now thinking about the real theory, the one with quark masses, 
the scale already enters decisively into fixing the 
bare quark masses in the Lagarangian, namely in planning the simulations.
Usually we do this by adjusting the pseudo scalar meson masses
to their physical values, since those are most sensitive to 
quark masses. The scale is needed for that. It is very important
to perform simulations at or close to the right quark mass, or 
on a given desired trajectory running through the physical point, 
in the parameter space given by the 
quark masses. For mass-degenerate u,d quarks, a  
trajectory may be given by fixed 
(physical or bare PCAC) strange 
(and ultimately charm quark) masses or for example
by a fixed trace of the quark mass matrix,  $\tr m_\quark = \rm const$.
In the past several collaborations missed the proper trajectory by more 
than what they would have liked to.

Furthermore, the scale enters where a momentum in a form factor
is fixed or into the overall size of the lattice. 
It is very useful to know the scale beforehand.
All of this calls for care in the selection and computation of the 
scale.


\subsubsection{What is a good scale?}
Unfortunately, the proton mass is not easily determined with good precision 
in lattice QCD computations due to a 
large noise/signal ratio in the proton correlation function,
see \sect{s:momega}.  The chiral scale $f$ is related to
experiments only through the chiral perturbation theory 
expansion. Consequently it is not common to use these
observables to set the scale. 
In general we should search for a quantity which\\  
{\vspace*{-1mm}
\bi \setlength{\itemsep}{0pt}
\item[(P1)]
is computable with a low numerical effort, 
\item[(P2)] 
has a good statistical precision,
\item[(P3)]
has small systematic uncertainties and
\item[(P4)]
has a weak quark mass dependence.
\ei
}
The first two properties are self explanatory, but 
the others require some details. By a good 
systematic precision we mean first of all that the
systematic error in the determination of the numbers
$M_i=a m_i$ for given bare coupling and quark masses is small.
For example such a systematic error may come from 
finite size effects or the contamination by excited states.
A second systematic uncertainty is the discretisation error. 
This is not easily judged. We will comment on it as we go along.
Concerning the quark masses, it is of course useful
to have a scale which depends weakly on them as this 
makes the tuning of the quark masses rather independent 
from the scale and, when the simulations are not at the physical point,
the extrapolation/interpolation to it is easier. Note that the
sensitivity to quark masses also depends on the trajectory 
one chooses to reach the physical point. For example the
mass of the Omega-baryon has a weak dependence on the light
quark masses when the strange quark mass is fixed, but not when
one is on the trajectory  $\tr m_\quark = \rm const$. On such a 
trajectory an appropriate average baryon mass has a weak quark-mass
dependence, see e.g. \cite{Cooke:2013qqa}.

For later use I define a measure 
for the quark mass dependence, 
$$
  \sm_{Q} = \frac{Q|_{\mpi=500~\MeV} - Q|_{\mpi=130~\MeV}}
      {Q|_{\mpi=130~\MeV}}\,,
      \label{e:sm}
$$
where $Q$ labels different scales, e.g. $Q=m_\prot$, and 
we assume that we are on a trajectory with strange and charm (bare, PCAC) mass 
fixed. Selfconsistently, MeV come from the scale 
$Q$. Since there is usually a rather linear dependence of
scales on $\mpi^2$, one has 
$\sm_Q \approx \frac{0.23~\GeV^2}{Q|_{\mpi=130~\MeV}}\frac{\partial Q}{\partial_{\mpi^2}}$. 

The statistical precision is determined both by the 
integrated autocorrelation time and by the variance.
These depend on the update algorithm and on the
chosen estimators, respectively. 
E.g. in the simplest case, using or not-using or stochastically-using
translation invariance are different estimators of a correlation function. 

 %{\cred xxx give a rating according to properties? xxx}

After this preparation, let me come to a discussion of a few 
scales which are in frequent use or newly proposed. I differentiate
between phenomenological scales
and theory scales. The former are related to physical
observables through a minimum amount of theory, while
the latter are constructed to be well computable in lattice
QCD but their values can (at present) only be 
computed in lattice QCD using a phenomenological scale
as an input. Thus a phenomenological scale is
needed in any case. The distinction between one category and the other 
is not sharp. For example I place $r_0$ \cite{Sommer:1993ce} with the 
theory scales, although (vague) phenomenological considerations
led to the prediction $r_0\approx 0.49$fm which is not far 
from our present knowledge.


\begin{table}[t!]
\begin{tabular}{lll lll | llllll } 
    \multicolumn{3}{c}{Wilson, $\Nf=2$} &
    \multicolumn{3}{c}{tmQCD,  $\Nf=2$} & 
    \multicolumn{4}{c}{$\Nf>2$} 
    \\
     $r_0$[fm] &  \multicolumn{2}{c}{from} & 
     $r_0$[fm] & \multicolumn{2}{c}{from} &
     $\Nf$ & $r_0$[fm] & $r_1$[fm] & \multicolumn{2}{c}{from} 
     \\[0.5ex] \hline \\[-1.5ex]
   $    0.503 (  10 ) $& $\fk$ & \cite{Fritzsch:2012wq} &      
   $    0.438 (  14 ) $& $\fk$ & \cite{Blossier:2009bx} &
   2+1 & $ 0.466(4)^a$ & $ 0.313(2)$ & div. & 
   \cite{Davies:2009tsa}
   \\
   $    0.491 (  ~6 )^c $& $\fk$ & \cite{Lottini:2013rfa} &&&&
      2+1 &  & $ 0.321(5)$ & $\Upsilon$ & \cite{Follana:2007uv}
\
   \\
   $    0.485 (  ~9 )^c $& $\fpi$ & \cite{Lottini:2013rfa}&    
   $    0.420 (  20 ) $& $\fpi$ & \cite{Baron:2009wt} %ETMC 08 from
   &
   2+1 & $0.470(4)$ & $0.311(2)$ & $\fpi$ & 
   \cite{Bazavov:2010hj,Bazavov:2011nk}
\\  
    $0.501(15)^b$    & $m_{\prot}$ & \cite{Bali:2012qs} &
   $    0.465 (  16 ) $& $m_{\prot}$ & \cite{Alexandrou:2009qu} 
   &   2+1 & $    0.492 (10)^b $ & & $m_\Omega$ & \cite{Aoki:2009ix} \\ 
   $    0.471 (  17) $& $m_\Omega$ &  &
     &&&
   2+1 & $    0.480 (  11 ) $ & $0.323(9)$ & $m_\Omega$ & \cite{Arthur:2012opa}\\ 
   &&& &&&
   2+1+1 & & 0.311(3) & $\fpi$ & \cite{Dowdall:2013rya} 
\\
\end{tabular}
\footnotesize
$^a$ with $r_0/r_1$ and $r_1/a$ from \cite{Bazavov:2009bb} 
\hspace*{2cm} $^c$ preliminary, at this conference
\\
$^b$ no continuum extrapolation
\caption{Values for $r_0,r_1$.  Column ``from'' shows the phenomenological scale 
used. All results except for those marked with $^b$ have been obtained by a
continuum extrapolation. 
\label{t:r0}}
\end{table}

\begin{table}[b!]
\begin{tabular}{llll} 
    $\nf$ & $\sqrt{t_0}$~[fm] & $w_0$~[fm]  & from\\[0.5ex] \hline \\[-1ex]
   0 &$   0.1638 (  10 ) $&$   0.1670 (  10 ) $& $r_0=0.49\,\fm$ \cite{Bruno:2013gha,Luscher:2010iy} \\ 
   2 &$   0.1539 (  12 ) $&$   0.1760 (  13 ) $& $\fk$ \cite{Bruno:2013gha,Lottini:2013rfa} \\ 
   3 &$   0.153~(7)         $&$   0.179~(6)         $& $m_\prot$\cite{lat13:roger} \\ 
   3 &$   0.1465 (  25 ) $&$   0.1755 (  18 ) $& $m_\Omega$ \cite{Borsanyi:2012zs} \\ 
   4 &$   0.1420 (   8 ) $&$   0.1715 (   9 ) $& $\fpi$ \cite{Dowdall:2013rya}\\ 
    \hline \\[-1ex]
\end{tabular}
\caption{Scales from the gradient flow. Note that these depend in principle
on the phenomenological scale they are determined from. 
\label{t:scales}
}
\end{table}
\clearpage


==> ScaleSetting/collaborations.tex <==
\subsection{Table of collaborations}

\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}  llrrr}
  Collaboration &  contact person   &   contacted & mail   & answer & read\\
  \hline
  \hline
  HPQCD & Christine Davies & 30 Oct/13 Nov & u & y\\
  \hline
  MILC & Alexei Bazavov, Urs Heller  & 30 Oct & u & y\\
  \hline
  Fermilab Lattice & Steven Gottlieb, James Simone & 30 Oct/13 Nov & u
  & y & cf. MILC\\
  \hline
  BMW & Christian Hoelbling & 30 Oct & u & y & r\\
  \hline
  ETMC & & 04 Nov & u & y\\
  \hline
  RBC/UKQCD & Andreas J & 30 Oct & r & y\\
  \hline
  ALPHA+CLS & Gunnar, Hartmut, Harvey& 29 Oct& r& y\\
  \hline
  QCDSF & Roger H & 30 Oct & r & y\\
  \hline
  PACS (PACS-CS) & Kuramashi & 30 Oct & r & y\\
  \hline
  HAL QCD & Aoki & 30 Oct & r & y\\
  \hline
  JLQCD & Shoji & 30 Oct & r\\
  \hline
  LHPC (?) & Orginos & 30 Oct & r & y\\
  \hline
  CALLAT & Walker-Loud & 30 Oct & r & y\\
  \hline
  PNDME & Rajan Gupta, Huey-Wen Lin& 30 Oct/13 Nov & u & y\\
  \hline
  HotQCD & Petretzky & 30 Oct & r & y\\
  \hline
  FlowQCD & Hiroshi Suzuki &  30 Oct & r & y\\
  \hline
  $\chi$QCD & Keh-Fei Liu & 30 Oct & u & y\\
  \hline
\end{tabular*}

\vspace*{2cm}

Here we list input received from collaborations.


BMW 2+1 \cite{Borsanyi:2012zs}, 1+1+1+1 \cite{Borsanyi:2012zs,Borsanyi:2020mff} \R
\\

RBC/UKQCD, 2+1: w0 and t0 "definite computation" \cite{Blum:2014tka}, "Contains scale determination in 2+1 QCD+QED but no explicit value for intermediate scales" \cite{Blum:2018mom} \N 
\\[1cm]

ALPHA + CLS \cite{Bruno:2016plf} +
possibly Mainz before deadline + (private emails to Rainer) Regensburg 
at end of 2020.
\\
HotQCD: $r_0, r_1$ \cite{Bazavov:2011nk}\\
Bazavov: $r_1, r_2$ \cite{Bazavov:2017dsy} \\
Qcdsf: unpubl paper\cite{Bornyakov:2015plz}, proceedings\cite{Bornyakov:2015eaa}


Callat: to come in Nov.

HAL QCD: no scale setting

PACS-CS: $r_0$ \cite{Aoki:2008sm}

MILC HISQ, 2+1+1 \\
On the HISQ ensemble we use an intermediate scale $f_{p4s}$, which is
ultimately determined from the PDG value of fpi.

The first determination was done in
A. Bazavov et al. (Fermilab Lattice and MILC Collaborations), \cite{Bazavov:2014wgs}
The latest result is \cite{Bazavov:2017lyh}
\\
t0 and w0 were determined in \cite{Bazavov:2015yea}
using the f{p4s} scale from \cite{Bazavov:2014wgs}\\



\subsubsection{mail by Christine D}

Further HPQCD references (with notes/remarks from Christine):\\
Toussaint and Davies \cite{Toussaint:2004cj} - first to point out the usefulness of the omega baryon mass for tuning QCD parameters on the lattice (but staggered baryon results at that time were not statistically accurate enough to provide competitive values compared to other methods). \\


A.~Gray et al \cite{Gray:2005ur} - first bottomonium spectrum calculation on gluon field configurations including sea quarks and demonstration of agreement with experiment(for the first time) 
Used $nf=2+1$ asqtad configs (with comparison to quenched and $nf=2$), NRQCD b quarks 
Determined $r_0$ and $r_1$ from the radial excitation energy in the Upsilon system ie M(2S)-M(1S) for Upsilon.
$r_0 = 0.469(7) \text{fm}, r_1 = 0.321(5) \text{fm}$ \\


CD et al \cite{Davies:2009tsa} - discussed and compared 3 different methods to determine the lattice spacing:\\ 
1) radial excitation energy in the Upsilon system (as above) \\
2) the mass difference between the $D_s$ meson and one half the $\eta_c$ meson. (More on this below) \\
3) the decay constant of the pseudoscalar s-sbar meson (related to experiment through its ratio to the combination of $2f_K - f_\pi$ at the physical point, determined in a lattice QCD calculation. This was the precursor to the MILC $f_{4ps}$ method (so you should cite this paper if/when discussing that method). \\
Using the $nf=2+1$ asqtad configurations, NRQCD b quarks for 1) and HISQ $c$ and light quarks for 2) and 3) this paper determined 
$r_1 = 0.3133(23)(3)$ fm. \\


R.~Dowdall et al. \cite{Dowdall:2011wh} - Improved bottomonium spectroscopy . Used improved NRQCD b quarks on the $nf=2+1+1$ gluon field configs. With HISQ sea quarks and also light meson decay constants with HISQ quarks. 
Found (section V) 
$r_1(\text{using} f_{\eta_s}) (\text{eq. 31}) = 0.3209(29)$ fm (this value is superseded in the paper below which did a better analysis). 
From the Upsilon splittings we had 
$_r1(\text{Upsilon}) = 0.310(6)$ fm \\



R.Dowdall et al \cite{Dowdall:2013rya} - full analysis of $f_K, f_pi$ and $f_{\eta_s}$ and including a determination of $w_0$ - the first accurate result for $w_0$ and first to use $f_\pi$. 
Used HISQ valence quarks on the $nf=2+1+1$ gluon field configs with HISQ sea quarks.
Found $w_0 = 0.1715(9)$ fm and, using ratios between $w_0$ and these other scales : 
$\sqrt(t_0) = 0.1420(8)$ fm, $r_1 = 0.3112(30)$ fm.
This value of $w_0$ is the one we have used since this paper i.e. it is our current value. \\


MILC HISQ, 2+1+1 \\
On the HISQ ensemble we use an intermediate scale $f_{p4s}$, which is
ultimately determined from the PDG value of fpi.

The first determination was done in
A. Bazavov et al. (Fermilab Lattice and MILC Collaborations), \cite{Bazavov:2014wgs}
The latest result is \cite{Bazavov:2017lyh}
\\
t0 and w0 were determined in \cite{Bazavov:2015yea}
using the f{p4s} scale from \cite{Bazavov:2014wgs}\\


Upcoming: D. Hatton et al, we are finalising and writing up a determination of $w_0$ using the mass difference between the $D_s$ and half the J/psi mass in QCD + quenched QED (i.e. updating and improving the method of 0910.1229). 
We think we should obtain an uncertainty of around 0.3\%. 
We obtain a result in good agreement with our previous value above and also BMW's number from earlier this year  

\subsection{double checks}
Rainer:

PACS-CS 08:  \good\bad\bad, text modifications 29.12.

Aubin 04: \soso\soso\soso, text modifications 29.12.

MILC 04: seems no new info compared to Aubin 04. removed.

\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{For completeness: $\Nf=2,0$}
ETMC, 2, clover: $t_0, t_0/w_0, w_0, r_0$  one lattice spacing at
physical point \cite{Abdel-Rehim:2015pwa} from $m_\pi, m_N, f_\pi,
f_K$
\\
flowQCD,0: \cite{Asakawa:2015vta}
\\
TWQCD: $N_f=2$ \cite{Chen:2014hva}




==> ScaleSetting/notes_Nazario.tex <==
\subsection{Nazario's Notebook}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{RBC/UKQCD 18 \cite{Blum:2018mom}}
\begin{itemize}

\item claim is first principles QCD+QED computation at physical pion mass of $a_\mu$ with non--degenerate up, down, strange and charm masses;

\item the charm is not dynamical, therefore this is a $1+1+1$ simulation;

\item the up, down and strange masses are fixed by using the \emph{experimental} values of the $\pi^0$, $\pi^+$, $K^0$ and $K^+$ masses (why four inputs for three quantities??) while the lattice spacing is set with the $\Omega^-$ mass. There are no plots or tables or anything useful to check these statements;

\item RM123 method by expanding around a $2+1$ QCD simulation with $m_{ud}$ and $m_s$ tuned by using $m_\pi=135.0$~MeV and $m_K=495.7$~MeV. The QED$_L$ prescription is used in the \emph{electroquenched approximation}.

\item meson masses are corrected for the universal $L^{-(1,2)}$ effects while $O(L^{-3})$ effects are declared to be ``small compared to statistical uncertainties''. Another tricky statement is ``The shift of the $\Omega^-$ mass due to QED corrections  is significantly smaller than the lattice spacing uncertainty and its effect is not included''. Again, no plots or tables or anything useful to check these statements;

\item in fact the QED effects are computed on a \emph{single} ensemble, the 48I of \cite{Blum:2014tka}, $a^{-1}=1.730(4)$~GeV. Moreover, they have only another ensemble, the 64I of \cite{Blum:2014tka}, $a^{-1}=2.359(7)$~GeV.

\item another ensemble is used to estimate charm contributions to $a_\mu$, this is taken from arXiv:1701.02644.

\item in summary, I don't think that is possible to extract from this paper any reproducible info concerning the lattice calibration procedure.
\\[1cm] 

\end{itemize}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{RBC/UKQCD 14 \cite{Blum:2014tka}}
\begin{itemize}

\item this is a gigantic paper corresponding to $2+1$ QCD simulations with domain--wall fermions;

\item in the abstract and introduction they say that use the \emph{physical} values of the pion, kaon and $\Omega$ mass (without the charges) to fix the light and strange quark masses and the scale;

\item the results $\sqrt{t_0}=0.7292\pm0.0041~GeV^{-1}$ and
$w_0=0.8742\pm0.0046~GeV^{-1}$ are first given in a table within the introduction;

\item the new ensembles generated in this work are Iwasaky+Shamir (32Ifine), Iwasaky+M\"obius (48I and 64I). The following figures come from TABLE II
\begin{eqnarray}
Size=\{48^3\times96\times24, 64^3\times128\times12, 32^3\times64\times12\}\;,
\nonumber \\
\nonumber \\
a^{-1}(GeV)=\{1.730(4),2.359(7), 3.148(17)  \}\;,
\nonumber \\
\nonumber \\
L(fm)=\{5.476(12),5.354(16), 2.006(1)  \}\;,
\nonumber \\
\nonumber \\
m_\pi L=\{3.863(6),3.778(8), 3.773(42)  \}\;.
\nonumber
\end{eqnarray}
The work also uses ensembles generated in previous works; 

\item the calculation of the $\Omega$ mass is discussed starting from pag.38; The plots in Figure~16 do not show a convincing plateaux, are fitted with two--exponentials on correlators with wall source and $Z_3$ source; The plots in Figure~17 on the stability of the mass wrt $t_{min}$ of the plateaux are a bit more convincing;

\item Wilson--flow scales are discussed starting from pag.41;

\item lattice calibration is discussed starting from pag.42;

\item the ``physical'' inputs are
\begin{eqnarray}
m_{\pi}=135.0~MeV\;,
\qquad
m_{K}=495.7~MeV\;,
\qquad
m_{\Omega}=1.67225~GeV\;.
\nonumber
\end{eqnarray}

\item results at the physical point are obtained with a combined continuum--chiral extrapolation with FVE corrected in ChPT or heavy--meson ChPT;

\item from TABLE~IX: the unitary pion mass is in the range $m_\pi^{unitary}\in[172,360]$~MeV; the lightest partially quenched pion mass is $144$~MeV.

\item the plot of the combined fit for the $\Omega$ mass is in Figure~22.

\item in the combined fit, the continuum extrapolation is done by including 6 ensembles with $a^{-1}=\{2.38, 2.36, 1.78, 1.73, 1.38, 3.15 \}$~GeV. In fact 4 different lattice spacings.

\item the final results for $w_0$ and $\sqrt{t_0}$ are given in eq.(73) and the plots for the continuum extrapolations are shown in Figure~26.

\end{itemize}


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{HotQCD 11 \cite{Bazavov:2011nk}}
\begin{itemize}

\item this is a paper on the QCD transition at finite temperature with $2+1$ dynamical fermions simulated using the p4, asqtad and HISQ actions and tree-level improved Symanzik gauge action;

\item the strange mass is required by imposing that the mass of a fictious $\eta_{s\bar s}$ meson is such that $m_{\eta_{s\bar s}}=\sqrt{2m_K^2-m_\pi^2}$ and then they interpolate to $m_l/m_s=0.037$ (where this comes from not stated immediately),  by simulating $m_l/m_s=\{0.2,0.1,0.05, 0.025 \}$.

\item zero temperature calculations are performed on ensembles with $m_\pi L> 2.6$ and as large as $m_\pi L=4.8$

\item the continuum extrapolation of $r_0/r_1$ is shown in Figure~3 and the best estimate for this quantity is $r_0/r_1=1.508(5)$.

\item the physical scale is than obtained by using the value $r_1=0.3106(8)(18)(4)$~fm obtained in \cite{Bazavov:2010hj} by the MILC collaboration by using $f_\pi$ to set the lattice spacing. This combined with their own determination of the ratio gives $r_0=0.468(4)$~fm.

\item the scale is also set by using $f_K$. In Figure~5 they show the continuum extrapolation for $f_\pi$, $f_K$ and $f_{\eta_{s\bar s}}$ in units of both $r_0$ and $r_1$ for the line of constant physics $m_l/m_s=0.05$ and compare with experimental values (with HPQCD for $f_{\eta_{s\bar s}}$). As far as I understand, the fact that they find agreement with experiment justifies both the use of chosen value of $r_1$ to set the scale and the fact that there is no significant effect in passing from $m_l/m_s=0.05$ to the physical value. The continuum extrapolations are in $a^2$. They have 20 ensembles at $m_l/m_s=0.05$ with lattice spacings in the range $[0.066,0.25]$~fm.

\item The interpolation to the physical value of $m_l/m_s$ is shown for thermodinamic observables but not for meson masses and decay constants. 

\item By using $f_K$ to set the scale their data for the chiral condensate show much smaller cutoff effects with repsect to the case of $r_1$.

\end{itemize}


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Bazavov 17 \cite{Bazavov:2017dsy}}

\begin{itemize}

\item 2+1 calculation of $T_c$ with HISQ quarks and tree-level improved Symanzik gauge action; extension of \cite{Bazavov:2014pvz} that is in Urs' list;

\item on the basis of previous experiences, they say that the quark mass dependence of the EoS is very small for $m_l<0.4 m_s$; therefore they use $m_l=0.2 m_s$ instead of the physical point; this corresponds to $m_\pi=320$~MeV.

\item the $T=0$ simulations have been performed at 5 different lattice spacings $a=\{0.025, 0.029, 0.035, 0.040, 0.082 \}$~fm.

\item at the smallest values of the lattice spacing they observe topology freezing and compare results in fixed topological sectors $Q=\{0,1,2\}$ to conclude that the effect is negligible on the observables of interest.

\item the scale is set by using $r_1$ and $r_2$ and the value $r_1=0.3106(8)(18)(4)$~fm obtained in \cite{Bazavov:2011nk} is taken.

\item for the two greatest lattice spacing they compare results with previous results at $m_l=m_s/20$ and asses that quark mass effects are of order $0.2\%$ for $r<r_1$ and in any case of the order of the statistical errors for distances of order $r_1$; this is shown in Figure~10. Building on this observation they quote results for $r_1/a$ and obtain $r_1/r_2 = 2.198(9)$. The continuum extrapolation is shown in Figure~11.

\end{itemize}



 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{MILC Asqtad 2+1}

%%%%%%%
\subsection*{MILC Asqtad 2+1 1: \cite{Aubin:2004wf}}

\begin{itemize}

\item simulations of Asqtad 2+1 fermions at two lattice spacings $a=\{0.09,0.12 \}$~fm, several quark masses down to $m_l/m_s=0.1$;

\item the dependence of $r_0/r_1$ as a function of $(m_\pi/m_\rho)^2$ is shown in Figure~1. These data are fitted simultaneously to the physical point and continuum limit; They obtain the value $r_0/r_1= 1.474(7)(18)$, eq.(5).

\item the physical value of the lattice spacing is then obtained by using the $\Upsilon$ 2S-1S and 1P-1S splittings determined with NRQCD in HPQCD~03 \cite{Wingate:2003gm}. From this they get $r_1=0.317(7)(3)$~fm corresponding to $r_1=1.606(35)(15)$~$GeV^{-1}$ and $r_0=0.462(11)(4)$~fm corresponding to $r_0=2.341(56)(27)$~$GeV^{-1}$. By using these numbers they get for the lattice spacings $a^{-1}=\{2.271(63), 1.588(19) \}$~GeV.

\item the physical values of the strange and quark masses are obtained by tuning $m_\pi$ and $m_K$ (the scale as before from the $\Upsilon$) but the explicit values of pion and kaon masses used as inputs are not quoted.

\item they write explicitly $m_\pi L=\{4.5, 6.3 \}$; at the smallest mass / coarser lattice I get $m_\pi L=3.8$ ($L/a=24$)

\item the lightest pion (difficult to find this info explicitly, I take data from Table~III) should be $m_\pi=336$~MeV on the finer--lighter lattice and $m_\pi=253$~MeV on the coarser--lighter lattice. 

\item 

\end{itemize}

%%%%%%%
\subsection*{MILC Asqtad 2+1 2: \cite{Aubin:2004fs}}

\begin{itemize}

\item this paper analyzes the same results of \cite{Aubin:2004wf} and extracts the following values for the decay constats in $1+1+1$ QCD
\begin{eqnarray}
f_\pi=129.5(0.9)(3.5)~MeV\;,
\qquad
f_K=156.6(1.0)(3.6)~MeV\;.
\nonumber 
\end{eqnarray}

\item they say that the lightest quark is such that $m_\pi/m_\rho\simeq 0.3$ corresponding to $m_\pi\simeq 250$~MeV. This does not correspond to my reading of the previous reference; It seems that in this paper they have another coarse ensemble with $m_l/m_s=1/10$. In fact two new ensembles, by using the data from Table~I I get indeed the 250~MeV pion mass that is such that $m_\pi L=3.8$.

\item maybe a typo, but here they quote $r_0/r_1= 1.472(7)$ instead of $r_0/r_1= 1.474(7)(18)$. Here, with the new ensemble they get $r_1=0.317(7)$~fm

\item the scale is set as described in the previous paper by using $\Upsilon$ spectrum. 2+1 QCD is defined by using as inputs 
%
\begin{eqnarray}
&&m_\pi=m_{\pi^0}=134.9768 MeV\;,
\nonumber \\
&&m_K=\sqrt{\frac{m_{K^0}^2+m_{K^+}^2-(1+\Delta_E)(m_{\pi^+}^2-m_{\pi^0}^2)}{2}}
= 494.374 MeV
\;,
\qquad
\Delta_E=1\;,
\nonumber
\end{eqnarray}
%
while 1+1+1 QCD is defined by using in addition to $m_K$ defined above also
%
\begin{eqnarray}
m_{K^+}= 493.677 MeV
\;.
\nonumber
\end{eqnarray}
%
\item {\cred Rainer: I see no new scale determination in that paper and would not mention it. I see no new ensembles compared to \cite{Aubin:2004wf}.\\ 
 I compare Table I of both papers.} Nazario: you are right, I was confused by a sentence saying that they have new ensembles but, in fact, with respect to an older paper. Therefore we can remove it!

\end{itemize}

%%%%%%%
\subsection*{MILC Asqtad 2+1 3: \cite{Bazavov:2009bb,Bazavov:2009fk,Bazavov:2009tw}}

\begin{itemize}

\item in \cite{Bazavov:2009bb} they extended the analysis of the previous papers by adding ensembles that cove now 6 different lattice spacings and $m_l~3m_{ud}$.

\item they have $a=\{ 0.045,0.06,0.09,0.12,0.15.0.18$~fm. On the three finer lattices $m_\pi L>4.1$; A nice summary is Figure~8.

\item in this paper they say that using the same two coarser lattices of \cite{Aubin:2004wf} they get $r_1=0.318(7)$~fm instead of $r_1=0.317(7)(3)$~fm. Maybe a typo maybe a small correction.

\item in this work, by setting the scale with $f_\pi$ (which value still to be understood) they get $r_1=0.3108(15)(+26)(-79)$~fm.

\item concerning spectroscopy, a nice summary is in Figure~15.

\item the results of the continuum and chiral extrapolations of the $\Omega$ mass are shown in Figure~20. But the number is not quoted here...

\item the schemes used to define 2+1 and 1+1+1 QCD are the same discussed in the previous subsection.

\item by using $r_1=0.318(7)$~fm they get
\begin{eqnarray}
f_\pi=128.3(0.5)(+2.4)(-3.5)~MeV\;,
\qquad
f_K=154.3(0.4)(+2.1)(-3.4)~MeV\;.
\nonumber 
\end{eqnarray}

\item by using $f_\pi^{exp}=130.7(0.1)(0.36)$ they get $r_1=0.3108(15)(+26)(-79)$~fm and $f_K=156.5(0.4)(+1.0)(-2.7)$~MeV.

\item in \cite{Bazavov:2009fk,Bazavov:2009tw} first appear the values of $m_\pi^{RMS}$. The lightest such pion has $m_\pi^{RMS}=258$~MeV, $m_\pi^{RMS} L>4.2$. in this proceeding they quote
\begin{eqnarray}
r_1^{\Upsilon}= 0.318(7) fm\;,
\qquad
f_\pi=128.0(0.3)(2.9)~MeV\;,
\qquad
f_K=153.8(0.3)(3.9)~MeV\;.
\nonumber 
\end{eqnarray}
while by using $f_\pi=130.4(0.2)$ to set the scale they get
\begin{eqnarray}
r_1= 0.3117(6)(+12)(-31) fm\;,
\qquad
f_\pi^{exp}=130.4(0.2)~MeV\;,
\qquad
f_K=156.2(0.3)(1.1)~MeV\;.
\nonumber 
\end{eqnarray}
 
\end{itemize}

%%%%%%%
\subsection*{MILC Asqtad 2+1 4: \cite{Bazavov:2011aa}}

\begin{itemize}

\item this is a paper on $f_B$ and $f_D$; the two finer ensembles are not used.

\item in this paper, the result $r_1= 0.3117(6)(+12)(-31)$~fm obtained in the previous subsection is averaged with the HPQCD result $r_1=  0.3133(23)(3)$~fm to get $r_1= 0.3117(22)$~fm.



\end{itemize}



 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{PACS-CS \cite{Aoki:2008sm}}

\begin{itemize}

\item 2+1 simulations of Clover Wilson fermions with Iwasaki gauge action.

\item single lattice spacing, $a=0.0907(13)$~fm on the volume $32^3\times 64$ and pion masses in the range $m_\pi\in [156,702]$~MeV. The lightest pion is such that $m_\pi L = 2.29$.

\item there is the explicit statement that the theory is calibrated by using $m_\pi$, $m_K$ and $m_{\Omega}$. I need now to understand the values. These are in Table~XI,
\begin{eqnarray}
m_{\pi}=135.0~MeV\;,
\qquad
m_{K}=497.6~MeV\;,
\qquad
m_{\Omega}=1.6725~GeV\;.
\nonumber
\end{eqnarray}

\item they quote $f_\pi=134.0(4.2)$ and $f_K=159.4(3.1)$ MeV.


\item plateux for the $\Omega$ correlators are shown in Figures~3,4,5,6. These are all quite convincing, including the case of the lighter pion. The interpolating operators are smeared and averaged over the polarization indexes (the four spin states for the decuplet barions): this apparently gives excellent plateauxs!!
{R: looks like luck to me. They use local-smeared effective masses and at higher pion mass the plateau is not so great. Anyway the analysis is ok. I am less sure for $V(r)$. N: we agree!}

\item $r_0$ is calculated at a single lattice spacing and chirally extrapolated and they get  $r_0=0.4921(64)(+74-2)$ fm .

\end{itemize}


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{QCDSF \cite{Bornyakov:2015eaa,Bornyakov:2015plz}}

%%%%%%%
\subsection*{proceeding: \cite{Bornyakov:2015plz}}

\begin{itemize}

\item 2+1 simulations, Iwasaki gauge action and stout--smeared Clover quarks.

\item expansion around the symmetric point $(2m_{ud}+m_s)/3$; the idea is that flavour singlet quantities have second order corrections in the expansion;

\item four lattice spacings, $m_\pi L >4$ with $m_\pi\in [220,500]$~MeV. 

\item the values of $w_0$ and $t_0$ are not quoted here, maybe in the paper.

\item I still don't understand what they do, certainly they take falvour $SU(3)$ symmetric combinations of pseudoscalar mesons, vector mesons and octect baryons masses. 

\item they ignore $O(\delta m_q^2)$ corrections and therefore these are functions only of the symmetric mass;

\item then they tune the symmetric mass by requiring that the ratio of two such quantities is equal to the physical values;

\item by taking one of these quantities than they set the lattice spacing

\item the previous reasoning is for two quantities and by neglecting $O(\delta m_q^2)$ I understand. then they say that they can "arrange" other two quantities to cross at the same value of the bare mass as before, how????

\end{itemize}

%%%%%%%
\subsection*{unpublished paper: \cite{Bornyakov:2015eaa}}


\begin{itemize}

\item ok I think we can call this 3 QCD and say that in the case of flavour $SU(3)$ symmetric quantities the approximation is not terribly bad.

\item in the paper, at pag.14 it seems that ``adjusting'' means that the lattice data have been multiplied for a factor to make the line cross at the same value of $k_0$... this does not make sense!!!

\item the value quoted are $\sqrt{t_0}=0.1511(22)(06)(05)(03)$~fm and $w_0=0.1808(23)(05)(06)(04)$~fm.

\end{itemize}






 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Double Checks}

%%%%%%%
\subsection{ETM 14}

chiral extrapolation: OK, \soso\\
continuum extrapolation: OK, \good\\
finite volume: OK, \good\\
quoted values: OK\\

%%%%%%%
\subsection{ETM 20}

chiral extrapolation: OK \good, $M_\pi^{min}$ and $M_\pi^{min} L$ not explicitly quoted but indirectly inferred by Urs\\
continuum extrapolation: OK \good\\
finite volume: OK \good\\
quoted values: OK\\

which flow? 

%%%%%%%
\subsection{MILC 15}

chiral extrapolation: OK \good\\
continuum extrapolation: OK \good\\
finite volume: OK \good\\
quoted values: OK\\

%%%%%%%
\subsection{HotQCD 14}

This is an extension of HotQCD11; They add 4 new values of $\beta$, for a total of 24 ensembles, and improve the statistic of the previous determinations; 

This meanse that they have lattice spacings in the range $[0.04,0.25]~fm$ and volumes in the range $[2.6,6.1]~fm$.

chiral extrapolation: I don't understand where the value $M_\pi^{min}=130$ MeV in Table 8 comes from, is this 160?? Should be \bad?\\
Strickly speaking, both $r_0/r_1$ and $w_0/r_1$ are obtained at fixed pion mass, $M_\pi^{min}=160$ MeV.
This is true also in HotQCDS11 but there they have simulations at more values of the pion mass. If we grade HotQCDS11 \good, then this also has to be \good, or vice versa for both the works.


continuum extrapolation: OK \good\\

finite volume: if I take $aM_\pi=0.03425$ from Table~V and N=64 from Table~III I get $M_\pi L= 2.2$. At the same time the same physical pion mass is simulated with $M_\pi L= 4.2$. This would imply \good \\
Yes it is good because they have a huge number of volumes.


quoted values: OK\\

which flow?



%%%%%%%
\subsection{RBC/UKQCD 10A}
continuum extrapolation: two lattice spacings $a^{-1}=\{1.73(3),2.28(3)$~GeV, \soso OK\\
chiral extrapolation: unitary pion masses in the range [290,420]~MeV, 3 pions at the finest and 2 at the coraser lattice spacings, \soso OK\\
finite volume: $m_\pi L=4.0$, this would imply \good\\
quoted values: OK


%%%%%%%
\subsection{$\chi$QCD 14}
continuum extrapolation: two lattice spacings $a^{-1}=\{1.75(4),2.33(5)$~GeV, the same ensembles of RBC/UKQCD 10A but slightly different figures because different determination of $r_0$, \soso OK\\
chiral extrapolation: 6 unitary pion masses, $m_\pi^{min}=290$~MeV, \soso, this differes from Urs!\\
finite volume: $m_\pi L=4.0$, this would imply \good\\
quoted value: OK

\newpage


==> ScaleSetting/notes_Urs.tex <==
\subsection{Notes by Urs}

{\bf MILC: \cite{Bazavov:2015yea}} \U
\begin{itemize}
\item $N_f=2+1+1$ highly improved staggered quarks, four lattice
  spacings $0.06 \text{ fm} \leq a \lesssim 0.15 \text{ fm}$ (0.15,
  0.12, 0.09, 0.06 fm),
  including physical quark masses
\item Symanzik flow, cloverleaf definition of energy density
  \item $M_\pi L$ can be inferred from Table I.
\item determination of $w_0 F_{p4s}$ and $\sqrt{t0} F_{p4s}$
    using previous determination of $F_{p4s}$ in physical units
    \cite{Bazavov:2014wgs}
\item  polynomial expansions to parametrize lattice-spacing effects
  instead of staggered chiral-perturbation theory in NNLO chiral extrapolation
\end{itemize}
\vspace*{1cm} 

{\bf HotQCD:  \cite{Bazavov:2014pvz}} \U
\begin{itemize}
\item determination of $r_0, r_1, w_0$  
\item simulations with $N_\tau=6, 8, 10, 12$ and spatial size
  $N_\sigma=4N_\tau$, temperature range $130 \text{MeV} \leq T \leq 400
  \text{MeV}$, using the highly improved staggered quark (HISQ)
action introduced by the HPQCD collaboration \cite{Follana:2006rc} completely
eliminate ${\cal O}(a^2)$ discretization errors at tree level
\item scale quantities can be found in Sec.II around eq.(1) and (2),
  details in App.B.
\item scales $r_0, w_0$ determined from continuum extrapolation of
  ratios $r_0/r_1, w_0/r_1$ and using $r_1 = 0.3106(14)(8)(4)$ fm
  from MILC 10 \cite{Bazavov:2010hj}
\item also measured the masses and decay constants
  of several light hadrons, providing
  further crosschecks on the scale setting in the continuum
  limit. Everything agrees, details in App.C.

\item Topological charge on the finest lattices $a~0.049, 0.041$ fm
  shows long autocorrelations of ${\cal O}(500 - 1000)$ trajectories,
  the latter covering only charges $\nu \in \{-1,+2\}$, cf. App.A.2
  (it's not clear which ensembles are shown).

\item for $\beta = 6.423$ they use $r_0$ to determine $r_1$ via
  $r_0/a/(r_0/r1)_{cont}$ to reduce lattice artefacts

\item in App.B they give $(w_0/r_1)_{cont} = 0.5619(21)$ or
    $w_0 = 0.1749(14)$ fm, no details on GF given.

\item they use $r_1 = 0.3106(14)(8)(4)$ fm from HPQCD 09B
  \cite{Davies:2009tsa} (check: earlier they refered to MILC 10
  \cite{Bazavov:2010hj} for the value).    
\item they also use $f_K$ to set the scale, cf. App.C, only as a
  crosscheck. The
cutoff dependence of $f_K$ and $m_\varphi$ is very similar to the cutoff dependence of $w_0$

\item zero-temperature lattice ensembles at 34 different
    $\beta$-values, line of constant physics fixed by $M_{\eta_{s\bar s}} = \sqrt{2 m_K^2 - m_\pi^2}$, $m_{ud} = m_s/20$
\item static potential from Coulomb gauge fixed confs and Coulomb-pluslinear-
  plus-constant potential fit form
\item $r_0/r_1$ appear to be independent of the lattice spacing
  within given uncertainties, so use constant extrapolation to continuum
\end{itemize}
\vspace*{1cm} 


{\bf ETMC, 2+1+1 non-clover: \cite{Carrasco:2014cwa}}  

\begin{itemize}
  \item $r_0$ at one lattice spacing, chiral
extrapolation, proceedings \cite{Baron:2008xa}, second lattice spacing
in proceedings \cite{Baron:2009zq}, paper \cite{Baron:2010bv}, three
lattice spacings in paper \cite{Carrasco:2014cwa}.
\item I look at the latest paper \cite{Carrasco:2014cwa}  only, because it supersedes the previous ones
\item Wilson TM fermions, Iwasaki gauge action 
\item unitary setup for the two light quarks and mixed action approach
  for the strange and charm quarks (OS valence fermions)
\item three lattice spacing $a=0.089, 0.082, 0.062$ fm
\item simulation parameters in Table 2, $211 \text{MeV} \leq M_\pi \leq 443 \text{MeV}$, $3.05 \leq M_\pi L \leq 5.4$.
\item $r_0/a$ calculated and extrapolated to the chiral limit at each $\beta$
\item lattice spacings set through $f_\pi=f_{\pi^+}=130.41$ MeV via intermediate scales $r_0$ and the fictitious pseudoscalar meson $M_{s's'}$ made of two strange-like
  quarks (cf.~procedures in next two items)
\item direct determination from $r_0 f_\pi$ at the physical point in the continuum using $f_\pi.$ 

\item convert $aM_{s's'}$ to $r_0 M_{s's'}$, then use $r_0/a$ in the chiral limit at each $\beta$, then continuum extrapolate $r_0 M_{s's'}$ and use $M_{s's'}$ determined from $f_\pi$,  cf.~3rd paragraph pg.19
\item chiral extrapolation uses ChPT and polynomial fits
\item $r_0 = (0.474\pm0.014)$fm in eq.(30), pg.21
\item chiral extrapolation crosschecked using $M_\pi < 400, 350, 300$ MeV instead of full range up to  $M_\pi < 450$ MeV
\end{itemize}
\vspace*{1cm} 


{\bf ETMC, 2+1+1 non-clover:\cite{Deuzeman:2012jw}} 

\begin{itemize}
\item $w_0$, three lattice spacings, no error
  given(!), proceedings 
\item result is noted in the text
\end{itemize}
\vspace*{1cm} 




{\bf ETMC, 2+1+1 clover: \cite{Alexandrou:2018egz}} 
\begin{itemize}
\item $t_0, w_0$ used but not determined, one lattice
spacing at physical point 
\item determination of the lattice spacing via the pion decay constant
and heavy quark observables, and 
determination of the lattice spacing via the nucleon mass.
\item summary of the different
determinations of lattice spacing via gluonic, mesonic and baryonic
observables in section 6.
\item uses $N_f=2+1+1$ Wilson twisted mass fermions at maximal twist
  Iwasaki improved gauge action

\item fermion action includes clover term with the clover parameter set by using an estimate from 1-loop tadpole boosted
perturbation theory
\item one lattice spacing, one pion mass only
\item extrapolate the GF observables to the chiral limit using a
  fit ansatz linear in $a \mu_\ell$, which corresponds to LO ChPT.
\item $t^{ch}_0/a^2 = 3.261(6)$ and ${w^{ch}_0}^2/a^2 =
  4.550(20)$, cf. section 6.
\item They use GF scales from BMWc to set the lattice spacing, but do
  not give physical values determined via $f_\pi$ and $m_N$.        
\item we do not need to follow this further
\end{itemize}
\vspace*{1cm} 


{\bf ETMC, 2+1+1 clover: \cite{Dimopoulos:2020eqd}} 
\begin{itemize}
\item $w_0$, three lattice spacings, physical point,
proceedings , paper to appear spring of 2021
\item uses $N_f=2+1+1$ Wilson twisted mass fermions at maximal twist Iwasaki improved gauge action
\item fermion action includes clover term with the clover parameter set by using an estimate from 1-loop tadpole boosted
  perturbation theory
\item three lattice spacings in the range $(0.10,0.07)$ fm
\item mixed action setup using Osterwalder-Seiler fermions in
    the valence $(c, s)$ quark sector
\item two ensembles at the physical point (however, pion masses are
  not given explicitly)
\item sea strange and charm quarks are set to values close to the
    physical ones (with a few percent tolerance)
\item imposing at physical point $M_\pi =134.8$ MeV, $f_\pi^{phen.}=130.41$ MeV yields $w_0=0.1706(18)$ fm from analyis of $f_\pi w_0$ in terms of $\xi_\ell^M = M_\pi^2/(16\pi^2 f^2)$
\item $w_0 = 0.1703(18)$ fm from analysis in terms of $\xi_\ell = 2B_0m_\ell/(16\pi^2 f^2)$
\end{itemize}
\vspace*{1cm}


{\bf $\chi$QCD 14: \cite{Yang:2014sea}}
\begin{itemize}
\item $N_f=2+1$ domain wall fermion configurations generated by the
  RBC/UKQCD Collaborations \cite{Aoki:2010dy} (Iwasaki gauge action)
\item two ensembles $24^3\times 64$ at $\beta=2.13$ and $32^3\times 64$ ate $\beta=2.25$, corresponding to $a=0.111$ and 0.083 fm.
\item residual quark masses are 0.00315(4) and 0.00067(1)
\item low-energy constant $\Delta_\text{mix}$ describing partial quenching effects is very small (cf. rmark 11 in their section III.A), mixed (light and valence quark) pion at $~300 MeV$ is shifted by $~10 MeV$
  \item quality rating for chiral extrapolation and finite volume taken over from RBC/UKQCD 10A in FLAG4 quark mass section. Note that LEC section has different FV rating (\bad instead of \good), LEC section quotes $M_{\pi,\text{min}} L = 2.7$, quark mass section 4.0
\end{itemize}
\vspace*{1cm}

{\bf RBC/UKQCD 10A \cite{Aoki:2010dy} }
\begin{itemize}
\item cf.~description in the text
\end{itemize}
\vspace*{1cm}


{\bf FNAL/MILC 17 \cite{Bazavov:2017lyh} }
\begin{itemize}
\item HISQ staggered fermions, 2+1+1 flavors, one-loop Symanzik and
tadpole improved gauge action
\item six lattice spacings from 0.15 fm down to 0.03 fm
\item minimum pion mass 131 MeV wih $M_\pi L=3.3$, cf. Table I, max. mass 329 MeV
\item experimental inputs corrected for e.m.~effects, cf.~table VI
\item for setting
the overall scale they use the pion decay constant $f_\pi = 130.50(13)$ MeV following PDG
\item $u,d,s$ quark masses from $M_\pi, M_K$, charm quark mass from $M_{D_s}$
\item they determine mass and decay constant of a fictitious pseudoscalar-meson with degenerate valence-quark masses $0.4 m_s$
\item $f_{p4s} = 153.98(11)(+2/-12)(12)[4]$ MeV, cf. section VIIB 
\item $M_{p4s} = 433.12(14)(+17/-6)(4)[40]$ MeV
\item ratio $f_{p4s}/M_{p4s} = 0.3555(3)(+1/-4)(3)[2]$ 
\end{itemize}
\vspace*{1cm}


{\bf FNAL/MILC 14A \cite{Bazavov:2014wgs} }
\begin{itemize}
\item HISQ staggered fermions, 2+1+1 flavors
\item four lattice spacings from 0.06 to 0.15 fm
\item minimum pion mass 130 MeV with $M_\pi L=3.7$, cf. Table I, max.~mass 349
  \item lattice spacing determined from $f_{\pi^+}$
  \item cf. Table VI for the values of $f_{p4s} = 153.90(9)(-15)(-02)(-05)(+14/-23)$, $M_{p4s} = 433.24(17)(-02)(-12)(-41)(+1/-33)$ and ratio $f_{p4s}/M_{p4s} = 0.35527(24)(-30)(+7)(+23)(+52/-15)$
\end{itemize}
\vspace*{1cm}






\subsubsection{Crosschecks}

{\bf Miller 20A: \cite{Miller:2020evg}}
\begin{itemize}
\item $N_f = 2+1+1$ highly improved, rooted
  staggered sea-quark (HISQ) configurations generated by the MILC and CalLat Collaborations
\item  M\"obius Domain-Wall fermions on GF smeared gauge fields in the valence sector (22 ensembles)
\item lattice spacings $0.06 \lesssim  a \lesssim 0.15$ fm, pion masses $130 \lesssim m_\pi \lesssim 400$ MeV
\item scale set using $m_\omega$, i.e., calculate $\sqrt{t_0} m_\Omega$ and $m_\Omega w_0$ on each ensemble
\item $\sqrt{t_0} = 0.1422(14)$ fm, $w_0 = 0.1709(11)$ fm (in abstract)
\item Symanzik flow and symmetric,
    cloverleaf definition of the field-strength tensor is used
  \item physicla point defined by $\bar M_\pi=134.8(3)$ MeV,  $\bar M_K=494.2(3)$ MeV, $\bar F_{\pi^+}=92.07(57)$ MeV, $\bar M_\Omega=1672.43(32)$ MeV  
  
\end{itemize}
\vspace*{1cm} 

  
{\bf BMWc 20: \cite{Borsanyi:2020mff}}
\begin{itemize}
\item $M_{\Omega_-} = 1672.45(29)$ MeV is used to set the scale, gives $w_{0,*} = 0.17236(29)(63)[70]$ fm (at physical point)
\item 4stout lattice action, i.e. tree-level Symanzik gauge action and a one-link staggered fermion
  action with four steps of stout smearing
\item 6 lattice spacings from 0.064 to 0.1315
\item $m_{\pi,\text{RMS}} = 155$ MeV at smallest lattice spacing
\item also uses 4HEX, $N_f=2+1$ one-link staggered quarks with four steps of HEX smeared gauge links, DBW2 gauge action for estimating FV effects
\item pion masses between 0.94-1.02 $M_{\pi,\text{phys}}^2$, i.e., 130.7 - 136.1 MeV
  \item certainly fullfils chiral criteria, but $m_{\pi,\text{min}} L$ difficult to estimate 
\end{itemize}
\vspace*{1cm}



{\bf HPQCD 13A:  \cite{Dowdall:2013rya}}
\begin{itemize}
\item Highly Improved Staggered Quark (HISQ) formalism and a fully
    ${\cal O}(\alpha_s a^2)$ improved gluon action
\item three values of lattice spacing, 0.15, 0.12, 0.09 fm
\item $f_\pi$ for over all scale setting
\item ratios $r_1/w_0 = 1.789(26)$ and $\sqrt{t_0}/w_0 = 0.835(8)$
\item they use $f_{\pi^+}, f_{K^+}$ and $m_{\pi^0}$ with isospin difference as error, i.e. $M_\pi^\text{phys}=134.98(32)$ MeV and $\sqrt{M_{K^+} M_{K^0}} = 494.6(3)$ MeV to fix quark masses
  \item they use $f_{\pi^+}=130.4(2)$ MeV for determining $w_0=0.1715(9)$ fm, cf. eq.(18), $\sqrt{t_0}=0.1420(8)$ fm and $r_1=0.3112(30)$ fm, cf. eq.(19)
\end{itemize}
\vspace*{1cm}


{\bf CLS 16:  \cite{Bruno:2016plf}}
\begin{itemize}
\item $N_f=2 + 1$ flavors of non-perturbatively $c_\text{SW}$-improved Wilson fermions with tree-level $O(a^2)$ improved Lu\"uscher-Weisz gauge action
\item three lattice spacings 0.085, 0.065, 0.05 fm
\item pion masses between 200 and 420 MeV
\item Using the experimental values of the meson masses corrected for isospin breaking
effects  and the PDG values for the decay constants, they use as input
parameters $m_\pi = 134.8(3)$ MeV ; $m_K = 494.2(3)$ MeV, $f_\pi = 130.4(2)$ MeV ; $f_K = 156.2(7)$ MeV
\item they give $\sqrt{8 t_0} = 0.415(4)(2)$ fm, corresponding to $\sqrt{t_0}=0.1467(14)(7)$ fm
\end{itemize}
\vspace*{1cm}


{\bf QCDSF/UKQCD 15:  \cite{Bornyakov:2015eaa}}
\begin{itemize}
\item $O(a)$ improved clover fermions, tree level Symanzik improved gauge action (?)
\item four lattice spacings 0.059, 0.068, 0.074, 0.082
\item simulations with the SU(3)-averaged quark mass kept constant
\item Wilson gradient flow, symmetrized clover definition for the action density
\item lowest pion mass 260 MeV (I get 230 MeV, with $M_\pi L = 4.10$ and $L=3.55$ fm)
  \item hadronic input is $X_\pi=0.4126$ GeV which correponds to SU(3) $(mass)^2$ averaged singlet quantity, and similarly $X_\rho = 0.8562, X_N=1.1610$ GeV 
  \item $\sqrt{t_0} = 0.1511(22)(06)(05)(03)$ fm, $w_0=0.1808(23)(05)(06)(04)$ fm
\end{itemize}
\vspace*{1cm}


{\bf BMW 12A:  \cite{Borsanyi:2012zs}}
\begin{itemize}
\item uses tw0 fermion discretizations: 2-stout staggered and 2-HEX Wilson-clover
\item scale set through $F_\pi$ and/or $M_\Omega$
\item interpolation to physical quark masses, pion masses down to 120 MeV, five lattice spacings, cf.\cite{Durr:2010aw} (numbers in appendix confirmed by Christain Hoelbling)
\item uses Wilson and Symanzik flow
\item $w_0 = 0.1755(18)(04)$ fm from Wilson fermions based on $M_\Omega$. \red{didn't find the value of $M_\Omega$ in physical units}
\end{itemize}
\vspace*{1cm}



{\bf HPQCD 11B:  \cite{Dowdall:2011wh}}
\begin{itemize}
\item HISQ action, tadpole-improved L\"uscher-Weisz gauge action
\item three lattice spacings
\item $\Upsilon 2S - 1S$ splitting to determine lattice spacing
\item $r_1 = 0.3209(26)$ fm
\end{itemize}
\vspace*{1cm}


{\bf HPQCD 09B:  \cite{Davies:2009tsa}}
\begin{itemize}
  \item based on MILC ensembles, tadpole-improved L\"uscher-Weisz
gauge action, HISQ staggered fermions (??)
\item $r_1 =0.3133(23)(3)$ fm through three different methods, $r_0 = 0.4661(38)$ fm from ratio of $r_0/r_1$ determined by MILC
\item 1) radial excitation energy in the $\Upsilon$ system $(m_\Upsilon - m_{\Upsilon'})$; 2) mass difference $m_{D_s} - m_{\eta_c}/2$; 3) ficticious decay constant $\eta_c$ (related to $f_{\pi,K}$)
\item five lattice spacings
\item using leading-order em/IB removed quantities for $m_\pi, m_K, f_\pi=0.1304(5)$ GeV, $f_K=0.1555(9)$
  \end{itemize}
\vspace*{1cm}

{\bf HPQCD 05B:  \cite{Gray:2005ur}}
\begin{itemize}
\item based on MILC ensembles, $r_{0,1}/a$ values taken from there (PRD 64, 054506 (2001), PRD70, 094505 (2004))
\item three coarse lattice spacings 0.09, 0.12, 0.17 fm
\item orbital $1P −1S$ (i.e. $1^1P_1−1^3S_1$) and radial
  $2S−1S$ (i.e. $2^3S_1−1^3S_1$) energy splittings are used for scale setting
\item $r_0=0.469(7)$fm, $r_1=0.321(5)$ fm
  \item lightest pion masses are 270, 360 and 330 MeV on the supercoarse, coarse and fine lattice spacing
\end{itemize}
\vspace*{1cm}




==> ScaleSetting/scalesetting_app_Nazario.tex <==
\newpage

\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 & \parbox[t]{4cm}{\centering 0.06, 0.08, 0.11, 0.14\\}& \parbox[t]{6.0cm}{Two versions of Domain Wall Fermions combined each with the Iwasaki gauge action} \\
HotQCD 11 & \cite{Bazavov:2011nk} & 2+1 & \parbox[t]{4cm}{\centering $[0.066,0.25]$\\}& \parbox[t]{6.0cm}{HISQ and tree-level improved Symanzik gauge action. Several ensembles with $a$ in the quoted range} \\
Aubin 04 & \cite{Aubin:2004wf} & 2+1 & \parbox[t]{4cm}{\centering 0.09, 0.12\\}& \parbox[t]{6.0cm}{Asqtad staggered quarks} \\
MILC 09 & \cite{Bazavov:2009bb,Bazavov:2009fk,Bazavov:2009tw} & 2+1 & \parbox[t]{4cm}{\centering $[0.045,0.18]$\\}& \parbox[t]{6.0cm}{Asqtad staggered quarks, 6 different lattice spacings in the quoted range} \\
PACS-CS 08 & \cite{Aoki:2008sm} & 2+1 & \parbox[t]{4cm}{\centering $0.09$\\}& \parbox[t]{6.0cm}{Several ensembles of Clover Wilson quarks and Iwasaki gauge action at a single lattice spacing} \\
[4.0ex] \hline \\[-1.0ex]
%
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in scale
  determinations with $N_f=2+1$, $N_f=2+1+1$ quark flavours.}
}
\end{table}



  
\begin{table}
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c l}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] &  $M_{\pi} L$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 &  $144$ & $3.9$ &  \parbox[t]{6.0cm}{The mass of the lightest unitary pion is 172~MeV}\\
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 &  $172$ & $3.8$ &  \parbox[t]{6.0cm}{The mass of the lightest unitary pion.}\\
%
HotQCD 11 & \cite{Bazavov:2011nk}    & 2+1 & $160$  & $4.8$ &  \parbox[t]{6.0cm}{HISQ staggered quarks, the pion mass quoted is $M_\pi$. Results on 20 ensebmles with volumes in the range $[3.2,6.1]~fm$, we quote $M_\pi^{min}L^{max}$. }\\
Aubin 04 & \cite{Aubin:2004wf}    & 2+1 & 253  & $3.8$ &  \parbox[t]{6.0cm}{Asqtad staggered quarks, the pion mass quoted is the goldstone mass}\\
MILC 09 & \cite{Bazavov:2009bb,Bazavov:2009fk,Bazavov:2009tw}    & 2+1 & 258  & $4.3$ &  \parbox[t]{6.0cm}{Asqtad staggered quarks, the pion mass quoted is $M_\pi^{RMS}$}\\
PACS-CS 08 & \cite{Aoki:2008sm} & 2+1 & 156  & $2.3$ &  \parbox[t]{6.0cm}{Clover quarks, several pion masses in the range $[156,720]$~MeV, single lattice spacing}\\
[4.0ex] \hline \\[-1.0ex]
%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline\\[-1.0ex]
%
\end{tabular*}
\caption{Chiral extrapolation \& finite-volume effects in scale determinations 
  with $N_f=2+1$ and $N_f=2+1+1$ quark flavours. We list the minimum pion mass $M_{\pi,\text{min}}$ and $M_{\pi} L$ at $M_{\pi} =M_{\pi,\text{min}}$.  }
}
\end{table}

\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


==> ScaleSetting/scalesetting_app_Rainer.tex <==
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
Miller 20A & \cite{Miller:2020evg} & 2+1+1 & 0.06, 0.09, 0.12, 0.15 & \parbox[t]{4.5cm}{M\"obius Domain-wall valence quarks on HISQ /  MILC sea}

\\[4.0ex] \hline \\[-1.0ex]
%
BMWc 20  & \cite{Borsanyi:2020mff} & 1+1+1+1 & 0.094, 0.078, 0.066, 0.055  & \parbox[t]{6.0cm}{Staggered fermion computation with Isospin breaking and QED}
\\[4.0ex] \hline \\[-1.0ex]
%
CLS 16  & \cite{Bruno:2016plf} & 2+1  & \parbox[t]{3cm}{\centering 0.05, 0.065, 0.085\\}& \parbox[t]{4.5cm}{NP O($a$) improved Wilson fermions with LW gauge action} \\
[4.0ex] \hline \\[-1.0ex]
% more than 3 pion masses w. 200<m,400
%
BMWc 12A  & \cite{Borsanyi:2012zs} & 2+1 & \parbox[t]{4.5cm}{0.092, 0.077, 0.065, 0.054 }  & \parbox[t]{6.0cm}{ Wilson fermion computation}
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 11B & \cite{Dowdall:2011wh} & 2+1+1 & 0.09, 0.12, 0.16 & \parbox[t]{4.5cm}{NRQCD for b-quark and HISQ for valence light quarks and MILC sea}
\\[4.0ex] \hline \\[-1.0ex]
%
MILC 10 & \cite{Bazavov:2010hj} & 2+1 & 0.045, 0.06, 0.09 & asqtad staggered quarks
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 09B &\cite{Davies:2009tsa} & 2+1 & 0.059, 0.084, 0.12, 0.15 &  \parbox[t]{4.5cm}{NRQCD for b-quark and HISQ for valence light quarks on MILC asqtad sea}
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 05B & \cite{Gray:2005ur} & 2+1 & 0.09, 0.12, 0.17 &  \parbox[t]{4.5cm}{NRQCD with tree level tadpole improved couplings on MILC asqtad sea}
\\[4.0ex] \hline \\[-1.0ex]
%
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in scale
  determinations with $N_f=2+1$, $N_f=2+1+1$ quark flavours.}
}
\end{table}


  \begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c l}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] &  $M_{\pi} L$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
Miller 20A & \cite{Miller:2020evg} & 2+1+1 & 130 & 3.9 & \parbox[t]{4.5cm}{M\"obius Domain-wall valence quarks on HISQ /  MILC sea}
\\[4.0ex] \hline \\[-1.0ex]
%
BMWc 20  & \cite{Borsanyi:2020mff} & 1+1+1+1 & 120  & 3.0 & \parbox[t]{6.0cm}{Staggered fermion computation with Isospin breaking and QED}
\\[4.0ex] \hline \\[-1.0ex]
%
CLS 16  & \cite{Bruno:2016plf}  & 2+1 & $200$  & 4.2 & \parbox[t]{6.0cm}{Extrapolation along line $m_u+m_d+m_s=\mathrm{const.}$} 
% Table I, D200 lattice.
\\[4.0ex] \hline \\[-1.0ex]
%
BMWc 12A  & \cite{Borsanyi:2012zs} & 2+1 & 120 \& 131 &  3.0 \& 3.9 & \parbox[t]{6.0cm}{Wilson fermion computation}
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 11B & \cite{Dowdall:2011wh} & 2+1+1 & 208 & 4.0 & NRQCD $\Upsilon$ 2s-1s splitting and $\eta_s$ as input
\\[4.0ex] \hline \\[-1.0ex]
%
MILC 10 & \cite{Bazavov:2010hj} & 2+1 & 170 & 4.8 & determination from global fit, scale from $f_\pi$
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 09B &\cite{Davies:2009tsa} & 2+1 & 260 & 3.9 & extension of HPQCD 05B  \cite{Gray:2005ur}
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 05B & \cite{Gray:2005ur} & 2+1 & 270 & 3.7 & NRQCD $\Upsilon$ 2s-1s splitting as input
\\[4.0ex] \hline \\[-1.0ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline \\[-1.0ex]
\end{tabular*}
\caption{Chiral extrapolation \& finite-volume effects in scale determinations 
  with $N_f=2+1$ and $N_f=2+1+1$ quark flavours. We list the minimum pion mass $M_{\pi,\text{min}}$ and $M_{\pi} L$ at $M_{\pi} =M_{\pi,\text{min}}$.  }
}
\end{table}
 

==> ScaleSetting/scalesetting_app_Urs.tex <==
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
BMWc 20   &  \cite{Borsanyi:2020mff} & 1+1+1+1 & \parbox[t]{3.5cm}{\centering 0.0640, 0.0787, 0.0952, 0.1116, 0.1191, 0.1315} &  \parbox[t]{5.5cm}{Staggered fermion computation with Isospin breaking and QED}  \\[4.0ex] 
\hline\\[-1.0ex]
%
Miller 20A & \cite{Miller:2020evg} & 2+1+1 & \parbox[t]{3.5cm}{$[0.056, 0.082, 0.11, 0.13]$, $[0.057, 0.087, 0.12, 0.15]$}   & \parbox[t]{5.5cm}{M\"obius Domain-wall valence quarks on HISQ /  MILC sea; lattice spacings depending on scheme} \\
[7.0ex] \hline \\[-1.0ex]
%
  ETM 20 & \cite{Dimopoulos:2020eqd} & 2+1+1 & 0.069, 0.079, 0.097 & \parbox[t]{5.5cm}{Wilson TM
  fermions at maximal twist including clover term. Note that  lattice spacings are not explicitely given in \cite{Dimopoulos:2020eqd}.}\\
  [9.0ex] \hline \\[-1.0ex]
%
ETM 18A & \cite{Alexandrou:2018egz} & 2+1+1 & 0.08 & \parbox[t]{5.5cm}{Wilson TM fermions at maximal twist including clover term}\\
  [4.0ex] \hline \\[-1.0ex]
%  
FNAL/MILC 17 &  \cite{Bazavov:2017lyh} & 2+1+1 &  \parbox[t]{3.5cm}{\centering 0.03, 0.042, 0.06, 0.09, 0.12, 0.15} & determination of $f_{p4s}$\\
[4.0ex]
\hline \\[-1.0ex]
%
MILC 15   & \cite{Bazavov:2015yea}  & 2+1+1 & \parbox[t]{3.5cm}{\centering 0.06, 0.09, 0.12, 0.15\\}& \parbox[t]{5.5cm}{Highly improved staggered quarks.} \\
[2.0ex] \hline \\[-1.0ex]
%
ETM 14 & \cite{Carrasco:2014cwa} & 2+1+1 & 0.089, 0.082, 0.062 & \parbox[t]{5.5cm}{Wilson TM fermions at maximal twist}\\
[2.0ex] \hline \\[-1.0ex]
%
FNAL/MILC 14A &  \cite{Bazavov:2014wgs} & 2+1+1 & 0.06, 0.09, 0.12, 0.15  & \\
[2.0ex]
\hline \\[-1.0ex]
%
HPQCD 13A &  \cite{Dowdall:2013rya} & 2+1+1 &  0.15, 0.12, 0.09 & \soso $\surd$(RS)\\
[2.0ex] \hline \\[-1.0ex]
%
HPQCD 11B &  \cite{Dowdall:2011wh} & 2+1+1 & 0.09, 0.12, 0.15 & \parbox[t]{5.5cm}{NRQCD for b-quark and HISQ for valence light quarks and MILC sea} \\
[4.0ex]
\hline \hline\\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in scale
  determinations with $N_f=2+1+1$ quark flavours.}
}
\end{table}




\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
CLS 16 & \cite{Bruno:2016plf} & 2+1 & 0.085, 0.065, 0.05 & \parbox[t]{5.5cm}{NP O($a$) improved Wilson fermions with LW gauge action} \\
[4.0ex] \hline \\[-1.0ex]
%
QCDSF/UKQCD 15 & \cite{Bornyakov:2015eaa} & 2+1 &  \parbox[t]{3.5cm}{\centering 0.059, 0.068, 0.074, 0.082} &  $(a_\text{max}/a_\text{min})=1.94$, \soso \\
[4.0ex]\hline \\[-1.0ex]
%
$\chi$QCD 14& \cite{Yang:2014sea} & 2+1 & 0.084, 0.112 & \parbox[t]{5.5cm}{Valence overlap fermions on domain wall fermion gauge configurations.}\\
[4.0ex] \hline \\[-1.0ex]
%
HotQCD 14 & \cite{Bazavov:2014pvz} & 2+1 & $[0.04,0.25]$ & \parbox[t]{5.5cm}{HISQ and tree-level improved Symanzik gauge action. Several ensembles with $a$ in the quoted range and with a single $M_\pi\approx 160\MeV$} \\[10.0ex]
\hline\\ [-1.0ex]
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 & \parbox[t]{3.5cm}{\centering 0.06, 0.08, 0.11, 0.14\\}& \parbox[t]{5.5cm}{Two versions of Domain Wall Fermions combined each with the Iwasaki gauge action} \\[7.0ex]
\hline\\ [-1.0ex]
%
BMW 12A &  \cite{Borsanyi:2012zs} & 2+1 & \parbox[t]{3.5cm}{\centering 0.053, 0.065, 0.077, 0.093} & \parbox[t]{5.5cm}{ Wilson fermion computation} \\
[4.0ex]\hline \\[-1.0ex]
%
HotQCD 11 & \cite{Bazavov:2011nk} & 2+1 & \parbox[t]{3.5cm}{\centering $[0.066,0.25]$\\}& \parbox[t]{5.5cm}{HISQ and tree-level improved Symanzik gauge action. Several ensembles with $a$ in the quoted range} \\[7.0ex]
\hline \\[-1.0ex]
%
RBC/UKQCD 10A &  \cite{Aoki:2010dy} & 2+1 & 0.087, 0.114 & \soso $\surd$ (RS) \\
[2.0ex]
\hline \\[-1.0ex]
%
MILC 10 & \cite{Bazavov:2010hj} & 2+1 & 0.045, 0.06, 0.09 & asqtad staggered quarks
\\[2.0ex] \hline \\[-1.0ex]
%
HPQCD 09B &  \cite{Davies:2009tsa} & 2+1 & \parbox[t]{3.5cm}{\centering 0.044, 0.059, 0.085, 0.12, 0.15} & \parbox[t]{5.5cm}{NRQCD for b-quark and HISQ for valence light quarks on MILC asqtad sea}
 \\
[4.0ex]\hline \\[-1.0ex]
%
MILC 09 & \parbox[t]{.5cm}{\cite{Bazavov:2009bb,Bazavov:2009fk,Bazavov:2009tw} }& 2+1 & \parbox[t]{3.5cm}{\centering $[0.045,0.18]$\\}& \parbox[t]{5.5cm}{Asqtad staggered quarks, 6 different lattice spacings in the quoted range} \\
[7.0ex]\hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2+1 & \parbox[t]{3.5cm}{\centering $0.09$\\}& \parbox[t]{5.5cm}{Several ensembles of Wilson clover quarks and Iwasaki gauge action at a single lattice spacing} \\
[7.0ex] \hline \\[-1.0ex]
%
HPQCD 05B &  \cite{Gray:2005ur} & 2+1 & 0.09, 0.12, 0.17  & \parbox[t]{5.5cm}{NRQCD with tree level tadpole improved couplings on MILC asqtad sea} \\
[4.0ex]\hline \\[-1.0ex]
%
Aubin 04 & \cite{Aubin:2004wf} & 2+1 & \parbox[t]{3.5cm}{\centering 0.09, 0.12\\}& \parbox[t]{5.5cm}{Asqtad staggered quarks}\\ [2.0ex]
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in scale
  determinations with $N_f=2+1$ quark flavours.}
}
\end{table}

  
\begin{table}
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c l}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] &  $M_{\pi} L$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
BMWc 20   &  \cite{Borsanyi:2020mff} & 1+1+1+1 &   \parbox[t]{2.75cm}{several pion masses within $\pm$3\% of physical value}  &  3.0   &       \\
[7.0ex] \hline\\[-1.0ex]
%
Miller 20A & \cite{Miller:2020evg}    & 2+1+1 &  130 & 3.9 &  \\
[2.0ex] \hline \\[-1.0ex]
%
ETM 20 & \cite{Dimopoulos:2020eqd} & 2+1+1 &  135 & 3.5 & \parbox[t]{5.5cm}{Only  indirectly inferred}\\
[2.0ex] \hline \\[-1.0ex]
%                      
  ETM 18A & \cite{Alexandrou:2018egz} & 2+1+1 &  139.8 & 3.6 & One ensemble only\\
[2.0ex] \hline \\[-1.0ex]
%                                                  
FNAL/MILC 17 &  \cite{Bazavov:2014wgs} & 2+1+1 & 129 & 3.7  & determination of $f_{4ps}, M_{4ps}$\\
[2.0ex]
\hline \\[-1.0ex]
%
MILC 15  & \cite{Bazavov:2015yea} & 2+1+1 & 125 & 3.7
%MILC 2015  & \cite{Bazavov:2015yea} & 2+1+1 & \parbox[t]{4.5cm}{$(2.4, 3.6,
%                                                4.8), (2.9, 3.8, 4.8,
%                                                5.8), (2.9, 4.3, 5.8),
%                                  (2.9, 3.8, 5.8)$} & $\gtrsim 3.3$ 
&  \parbox[t]{5.5cm}{Four ensembles at physical point.}\\
[2.0ex] \hline \\[-1.0ex]
%
ETM 14 & \cite{Carrasco:2014cwa} & 2+1+1 & 211 & 3.19 &\\
[2.0ex] \hline \\[-1.0ex]
%
FNAL/MILC 14A &  \cite{Bazavov:2014wgs} & 2+1+1 & 130 & 3.7 & determination of $f_{4ps}, M_{4ps}$\\
[2.0ex]
\hline \\[-1.0ex]
%
HPQCD 13A &  \cite{Dowdall:2013rya} & 2+1+1 & 128 & 3.7 & \good $\surd$(RS)\\
[2.0ex] \hline \\[-1.0ex]
%
HPQCD 11B & \cite{Dowdall:2011wh} & 2+1+1 & 211 & 4.0 & \parbox[t]{5.5cm}{NRQCD $\Upsilon$ 2s-1s splitting and $\eta_s$ as input}
\\[4.0ex] \hline\hline \\[-1.0ex]
%
%HPQCD 11B &  \cite{Dowdall:2011wh} & 2+1+1 & 220 & 4.3 & \soso\\
%[2.0ex]\hline\hline \\[-1.0ex]
%
\end{tabular*}
\caption{Chiral extrapolation \& finite-volume effects in scale determinations 
  with $N_f=2+1+1$ quark flavours. We list the minimum pion mass $M_{\pi,\text{min}}$ and $M_{\pi} L \equiv M_{\pi,\text{min}} [L(M_{\pi,\text{min}})]_\text{max}$ is evaluated at the maximum value of $L$ available at $M_{\pi} =M_{\pi,\text{min}}$.  }
}
\end{table}





\begin{table}
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c l}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] &  $M_{\pi} L$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
CLS 16 & \cite{Bruno:2016plf} & 2+1 & 200 & 4.2 & \parbox[t]{5.0cm}{Extrapolation along line $m_u+m_d+m_s=\mathrm{const.}$} \\
[4.0ex] 
\hline\\[-1.0ex]
%
QCDSF/UKQCD 15 & \cite{Bornyakov:2015eaa} & 2+1 & 230 & 4.1 & \soso \\
[2.0ex]
\hline\\[-1.0ex]
%
$\chi$QCD 14& \cite{Yang:2014sea} & 2+1 & 290 & 4.0 & \parbox[t]{5.0cm}{}\\
[2.0ex] \hline \\[-1.0ex]
%
HotQCD 14 & \cite{Bazavov:2014pvz} & 2+1 & 160 & 4.8 & \parbox[t]{5.0cm}{HISQ staggered quarks, the pion mass quoted is $M_\pi$. Results on 20 ensembles with volumes in the range $[2.6,6.1]$~fm, we quote $M_\pi^{min} L^{max}$.}\\ 
[12.0ex]\hline \\[-1.0ex]
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 &  $144$ & $3.9$ &  \parbox[t]{5.0cm}{The mass of the lightest unitary pion is 172~MeV}\\
[4.0ex] 
\hline\\[-1.0ex]
%
RBC/UKQCD 14  & \cite{Blum:2014tka}  & 2+1 &  $172$ & $3.8$ &  \red{\parbox[t]{5.0cm}{The mass of the lightest unitary pion.}}\\
[4.0ex] 
\hline\\[-1.0ex]
%
BMW 12A &  \cite{Borsanyi:2012zs} & 2+1 &  131 and 120 & 3.92 and 3.0 & \\
[2.0ex]\hline \\[-1.0ex]
%
HotQCD 11 & \cite{Bazavov:2011nk}    & 2+1 & $160$  & $4.8$ &  \parbox[t]{5.0cm}{HISQ staggered quarks, the pion mass quoted is $M_\pi$. Results on 20 ensembles with volumes in the range $[3.2,6.1]$~fm, we quote $M_\pi^{min}L^{max}$. }\\
[12.0ex]
\hline \\[-1.0ex]
%
RBC/UKQCD 10A &  \cite{Aoki:2010dy} & 2+1 & 290 & 4.0 & \\
[2.0ex]
\hline \\[-1.0ex]
%
MILC 10 & \cite{Bazavov:2010hj} & 2+1 & 170 & 4.8 & \parbox[t]{5.0cm}{determination from global fit, scale from $f_\pi$}
\\[4.0ex] \hline \\[-1.0ex]
%
HPQCD 09B&  \cite{Davies:2009tsa} & 2+1 & 211 & 4.0 & extension of HPQCD 05B  \cite{Gray:2005ur}\\
[2.0ex]\hline \\[-1.0ex]
%
MILC 09 & \parbox[t]{.5cm}{\cite{Bazavov:2009bb,Bazavov:2009fk,Bazavov:2009tw}}    & 2+1 & 258  & $4.3$ &  \parbox[t]{5.0cm}{Asqtad staggered quarks, the pion mass quoted is $M_\pi^{RMS}$}\\
[7.0ex]\hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2+1 & 156  & $2.3$ &  \parbox[t]{5.0cm}{Clover quarks, several pion masses in the range $[156,720]$~MeV, single lattice spacing}\\
[7.0ex]\hline \\[-1.0ex]
%
HPQCD 05B & \cite{Gray:2005ur} & 2+1 & 270 & 3.7 & NRQCD $\Upsilon$ 2s-1s splitting as input\\
[2.0ex]\hline \\[-1.0ex]
%
Aubin 04 & \cite{Aubin:2004wf}    & 2+1 & 253  & $3.8$ &  \parbox[t]{5.0cm}{Asqtad staggered quarks, the pion mass quoted is the Goldstone mass}\\
[4.0ex]
%
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Chiral extrapolation \& finite-volume effects in scale determinations 
  with $N_f=2+1+$ quark flavours. We list the minimum pion mass $M_{\pi,\text{min}}$ and $M_{\pi} L \equiv M_{\pi,\text{min}} [L(M_{\pi,\text{min}})]_\text{max}$ is evaluated at the maximum value of $L$ available at $M_{\pi} =M_{\pi,\text{min}}$.  }
}
\end{table}
 

% HotQCD 14 numbers:
% 
% Table IV:
% ------------------------------------
% 6.050 2.194(22) 1.440(31)  1.524(36)
% 6.100 2.289(21) 1.522(30)  1.504(33)
% 6.341 2.939(11) 1.935(30)  1.519(24)
% 6.950 5.249(20) 3.485(22)  1.506(11)
% 7.030 5.691(32) 3.763(13)  1.512(10)
% 
% 5.900 1.909(11) 1.230(133) 1.552(168)
% 6.000 2.094(21) 1.386(80)  1.511(89)
% 6.195 2.531(24) 1.670(30)  1.516(31)
% 6.285 2.750(30) 1.822(30)  1.509(30)
% 6.354 2.986(41) 1.959(30)  1.524(31)
% 6.423 3.189(22) 2.096(21)  1.522(18)
% 6.460 3.282(32) 2.165(20)  1.516(20)
% 6.488 3.395(31) 2.235(21)  1.519(20)
% 6.550 3.585(14) 2.369(21)  1.513(15)
% 6.608 3.774(20) 2.518(21)  1.499(15)
% 6.664 3.994(14) 2.644(23)  1.511(14)
% 6.740 4.293(32) 2.856(11)  1.503(13)
% 6.800 4.541(30) 3.025(22)  1.501(15)
% 6.880 4.959(28) 3.265(23)  1.519(14)
% 7.150 6.299(59) 4.212(42)  1.495(20)
% 7.280 7.140(53) 4.720(33)  1.513(15)
% 7.373 7.801(79) 5.172(34)  1.508(18)
% 7.596 9.443(237 6.336(56)  1.490(40)
% 7.825 11.51(378 7.690(58)  1.497(50)
% 
% Table V:
% -------------------------------------------------------
% 6.515 0.10975 (12) 0.34453(29) 0.47516(29)
% 6.575 0.10469 (68) 0.32521(55) 0.44869(50)
% 7.030 0.06744 (15) 0.21202(19) 0.29381(20)
% 
% 5.900 5.900 5.900  0.20162 (09) 0.63407(17) 0.86972(11)
% 6.000 6.000 6.000  0.18381 (37) 0.57532(51) 0.79046(27)
% 6.195 6.195 6.195  0.15143 (14) 0.47596(16) 0.65506(11)
% 6.285 6.285 6.285  0.13823 (50) 0.43501(47) 0.59951(28)
% 6.354 6.354 6.354  0.12923 (15) 0.40628(20) 0.55982(17)
% 6.423 6.423 6.423  0.12022 (12) 0.37829(19) 0.52161(17)
% 6.460 6.460 6.460  0.11528 (21) 0.36272(34) 0.50137(32)
% 6.488 6.488 6.488  0.11245 (15) 0.35313(27) 0.48716(17)
% 6.550 6.550 6.550  0.10629 (16) 0.33322(38) 0.45989(24)
% 6.608 6.608 6.608  0.10001 (17) 0.31333(28) 0.43286(29)
% 6.664 6.664 6.664  0.09572 (18) 0.29837(37) 0.41178(32)
% 6.740 6.740 6.740  0.087991(64) 0.27735(12) 0.38342(10)
% 6.800 6.800 6.800  0.0849  (18) 0.26387(99) 0.36257(68)
% 6.880 6.880 6.880  0.07714 (16) 0.24314(16) 0.33630(11)
% 7.150 7.150 7.150  0.06126 (18) 0.19231(20) 0.26631(16)
% 7.280 7.280 7.280  0.05516 (17) 0.17209(19) 0.23824(18)
% 7.373 7.373 7.373  0.04990 (22) 0.15530(16) 0.21531(12)
% 7.596 7.596 7.596  0.04106 (44) 0.12896(30) 0.17810(12)
% 7.825 7.825 7.825  0.03425 (23) 0.10695(46) 0.14731(15)
% 
% Table III:
% ----------
% 5.900  24
% 6.000  24
% 6.195  32
% 6.285  32
% 6.354  32
% 6.423  32
% 6.460  32
% 6.488  32
% 6.550  32
% 6.608  32
% 6.664  32
% 6.740  48
% 6.800  32
% 6.880  48
% 7.150  48
% 7.280  48
% 7.373  48
% 7.596  64
% 7.825  64
% 
% Lovera={
% 24,
% 24,
% 32,
% 32,
% 32,
% 32,
% 32,
% 32,
% 32,
% 32,
% 32,
% 48,
% 32,
% 48,
% 48,
% 48,
% 48,
% 64,
% 64}
% 
% 
% 
%   
% 
% r1ova={1.230,
% 1.386,
% 1.670,
% 1.822,
% 1.959,
% 2.096,
% 2.165,
% 2.235,
% 2.369,
% 2.518,
% 2.644,
% 2.856,
% 3.025,
% 3.265,
% 4.212,
% 4.720,
% 5.172,
% 6.336,
% 7.690}
% 
% aMpi={0.20162,
% 0.18381,
% 0.15143,
% 0.13823,
% 0.12923,
% 0.12022,
% 0.11528,
% 0.11245,
% 0.10629,
% 0.10001,
% 0.09572,
% 0.08799,
% 0.0849 ,
% 0.07714,
% 0.06126,
% 0.05516,
% 0.04990,
% 0.04106,
% 0.03425};

